Differentially Private Data Release via Statistical Election to Partition Sequentially

Differential Privacy (DP) formalizes privacy in mathematical terms and provides a robust concept for privacy protection. DIfferentially Private Data Synthesis (DIPS) techniques produce and release synthetic individual-level data in the DP framework. One key challenge to developing DIPS methods is preservation of the statistical utility of synthetic data, especially in high-dimensional settings. We propose a new DIPS approach, STatistical Election to Partition Sequentially (STEPS) that partitions data by attributes according to their importance ranks according to either a practical or statistical importance measure. STEPS aims to achieve better original information preservation for the attributes with higher importance ranks and produce thus more useful synthetic data overall. We present an algorithm to implement the STEPS procedure and employ the privacy budget composability to ensure the overall privacy cost is controlled at the pre-specified value. We apply the STEPS procedure to both simulated data and the 2000-2012 Current Population Survey youth voter data. The results suggest STEPS can better preserve the population-level information and the original information for some analyses compared to PrivBayes, a modified Uniform histogram approach, and the flat Laplace sanitizer.

==> old/comments.tex <==

Key issues with the paper are that (1) the proposed method is very similar to existing methods, which are not cited in the paper, and which have been found suboptimal under some circumstances (see Reviewer); (2) the writing is difficult to follow for any audience; sometimes too much knowledge is assumed, whereas at others very basic concepts are explained (see also Reviewer comments); and (3) the comparison of the methods is insufficient, because differences can easily occur due to random chance and a different table showing opposite conclusions could well be produced from some other chance draw. Instead, the authors should show the distribution of coefficients over the mechanism.


Referee: 1

Comments to the Author
 It also claims that it provides some other novel results such as SPECKS metric. However, there is a significant oversight of the available literature of a number of algorithms directly comparable to theirs and on the metrics to compare synthetic and the original data. There are likely technical flaws as well. Paper is also rather difficult to read in its current form. 


Abstract: What does this mean? "...per their differentiability of the data variability."


INTRO: 

DIPS is a technique that has some merit but a number of technical issues that have not been properly explained in published literature to my knowledge. In particular, the DIPS methods of the same authors upon which the proposed STEPS in part builds on (in addition to the UH algorithm) is only available in the Arixiv papers from 2016 --Yet the authors refer to those as something that sounds like well-established methods. 

Pg. 3 all kinds of refs are missing especially on utility; please see further. 

line 39 "to synthize" or "synthizer" 

line 39: This is a wrong statement! Karwa et al. (2017) proposed a local DP method (Duchi et al. 2013) synthesize the edges in social network data and designed a Markov Chain Monte Carlo method to incorporate the local DP mechanism explicitly to obtain posterior inferences. -- Karwa et al do NOT do local DP as defined by Duchi. A randomized response with DP is not in general equal to local DP! Karwa et al do the usual epsilon-DP but for the edges of the networks

line 54: "best out of the differentially private hierarchical histogram methods." Best in which way? With respect to what? Is it only L1 distance which is what most often is reported in the CS literature or something else?

In general I think that there should be a bit more critical review of some of these papers, at least a few more substantial statements regrading their pluses and minuses. 

page 4, line 7: "specific DP mechanisms. " You do NOT mention in the previous page when you recall some of the methods, with respect to which DP mechanism they work. Are they all Laplace mechanism and all epsilon-DP or are they some variants including e,delta-DP and/or Gaussian or geometric, etc...?

page 4, line 14: "
14 dimensionality reduction and model selection procedure will be needed, likely based on a 15" OK so are these also done in a DP-way? If not, then the whole product is not necessarily fully DP and this has to be stated clearly. There is a paper on model selection; see Lei et all JRSS 2018 I think. 

You are working with sequentially modeling of the full joint distribution and adding noise to both the marginal and conditional distributions, or rather functions of those. This has been done before and you identify some papers but not a few additional ones that are very similar to what you are doing. For example see PrivBayes algorithm or Li et al. 2018 in JPC. The latter I think even shows some issues with the PrivBayes when the noise is added to the conditional distributions similar in a manner you describe. 

pag 4, lines 34-36 ... I don't know what I am supposed to get from this sentence. I still don't understand what you mean by statistical differentiability, or the order of decomposition is determined per a statistical procedure. Maybe you can at least give one hint or simple example or point the reader where you define these terms.

pg. 4. line 44: How does this new metric compare to already established metrics, e.g., Snoke et al 2017 JRSS on utility for synthetic data, and within DP context Snoke and Slavkovic 2018 on pMSE mechanism. How does your procedure which essentially works via trees compares to the CART of Snoke and of his proposed measure for the quality of the synthetic DP data? In particular these measure are also based on propensity scores. I feel then you need to provide some review of such measures already existing  the SDC literature. 

pg 5, line 55 "... is low as with our without ..." This doesn't read well. I know what you are trying to say but please complete the sentence for readability. 


page 6, 2nd par -- I think you should add a comment here that contrast release of multiple statistics under DP from releasing g such stats form synthetic DP data. Which you do in the last paragraph of the subsection. So I would suggest that you move up all defs together at the start of sec 2.1., and then provide those insightful comments

page 6. There are many other works discussing different norms, including l-infinity, for GS! (e.g., see Awan work or Ulhman's work). I  find it problematic that the only paper referenced on this topic is an unpublished paper by one of the co-authors, while clearly there are others. 


Sec 2.2., Again, How about PrivBayes, and/or JPC paper by Li et al? ...

page 9, line 42. If I understand this, then choosing different L in a non-DP way will then lead to the entire procedure not being really epsilon-DP. This is a common problem, and many other papers have suggested that some optimal parameter exists and it's not chosen in a DP way but the comment about this needs to be made explicit. I think that some of the paprs you have not referenced, explicitly talk about this. 


Sec 2.3 Again this is where there has been work done on building off S&R and proposing propensity like measures to evaluate synthetic and original data. So there is not much new here. You need to evaluate the current literature! 

Section 3. It's has been show that Laplace is not an idea noise for categorical data like this. You are much better off with trying discrete Laplace, geometric etc... So not sure how fair comparison this is. Furthermore, many algorithms propose synthetic for categorical data. 

pg 12. line 14. "the loglinear model". Which one? You fitted all main effect, two-way interactions...???

This is very sparse contingency table! How well can you trust the AIC from the log-linear models fitted? How well do you preserve the zeros? Many of the DP synthetic histogram type algorithms have a problem with this. 

Feasability: Sec 3.3. The fact that Laplace does comparable to your method is not very encouraging. What do you gain by your method then really when you get as much with the much simpler algorithm? Although I do agree that you do  a bit better on the logistic regression. 

Table 5 and Table 6. Why do you need Table 5? Why not report the point estimates with their sign in Table 6?

Sec 4. If the strength of your proposed algorithm is the generation of DP synthetic data regardless of the variable type, than I think you should provide another example where you could show improvement over other types.

